The effect of smooth parametrizations on nonconvex optimization landscapes

We develop new tools to study landscapes in nonconvex optimization. Given one optimization problem, we pair it with another by smoothly parametrizing the domain. This is either for practical purposes (e.g., to use smooth optimization algorithms with good guarantees) or for theoretical purposes (e.g., to reveal that the landscape satisfies a strict saddle property). In both cases, the central question is: how do the landscapes of the two problems relate? More precisely: how do desirable points such as local minima and critical points in one problem relate to those in the other problem? A key finding in this paper is that these relations are often determined by the parametrization itself, and are almost entirely independent of the cost function. Accordingly, we introduce a general framework to study parametrizations by their effect on landscapes. The framework enables us to obtain new guarantees for an array of problems, some of which were previously treated on a case-by-case basis in the literature. Applications include: optimizing low-rank matrices and tensors through factorizations; solving semidefinite programs via the Burer-Monteiro approach; training neural networks by optimizing their weights and biases; and quotienting out symmetries.

==> character_of_props.tex <==
\section{Characterizations of lift properties}\label{sec:characters}
We now characterize the above properties. The characterization of {\localimplieslocal} below is easy to state.
\begin{theorem} \label{thm:localimplocalcharact}
	Let $x = \varphi(y)$.
	The lift $\varphi \colon \calM \to \calX$ satisfies the {\localimplieslocal} property at $y$ if and only if it is open at $y$.
	Globally, the lift $\varphi$ satisfies the {\localimplieslocal} property if and only if it is open.
\end{theorem}
Proving that openness is sufficient for {\localimplieslocal} is easy.
Proof of its necessity requires substantial work, deferred to Appendix~\ref{apdx:liftsopen}.
Our proof in the appendix provides the result in a more general, topological setting without using smoothness.
Moreover, it provides (possibly new) conditions which are equivalent to openness and may be easier to check in some situations. 

To characterize the {\oneimpliesone} and {\twoimpliesone} properties, we need to consider velocities and accelerations of curves on $\calX$ obtained by pushing curves on $\calM$ through the lift $\varphi$. To that end, we introduce the following definitions.
\begin{definition}\label{def:LQ_maps}
    Let $\varphi\colon\calM\to\calX$ be a smooth lift and fix $y\in\calM$. For each $v\in \T_y\calM$, choose a curve $c_v$ on $\calM$ satisfying $c(0)=y$ and $c'(0)=v$. Define maps $\Lmap_y, \Qmap_y\colon\T_y\calM\to\calE$ by
    \begin{equation*}
        \Lmap_y(v) = (\varphi\circ c_v)'(0),\qquad \Qmap_y(v) = (\varphi\circ c_v)''(0).
    \end{equation*}
    We write $\Lmap_y^{\varphi}$ and $\Qmap_y^{\varphi}$ when we wish to emphasize the lift.
\end{definition}
Of course, $\Lmap_y$ is simply the differential $\D\varphi(y)$, and is therefore linear and independent of the choice of curves $c_v$. The value of $\Qmap_y(v)$ does depend on the choice of $c_v$ but, importantly, this is inconsequential for our purposes: see Remark~\ref{rmk:nonunique_Q}. We explain how to compute $\Lmap_y$ and $\Qmap_y$ without explicitly choosing curves $c_v$ in Section~\ref{sec:Qmap_comp}.

Our characterization of {\oneimpliesone} can now be concisely stated.
\begin{theorem}\label{thm:oneimpliesone_char}
$\varphi$ satisfies {\oneimpliesone} at $y\in\calM$ if and only if $\im\Lmap_y = \T_x\calX$, where $x=\varphi(y)$.
\end{theorem}
We further show that if $\varphi$ satisfies {\oneimpliesone} at $y$ and $x=\varphi(y)$ is a smooth point of $\calX$, that is, $\calX$ is a smooth embedded submanifold of $\calE$ near $x$, then $\varphi$ satisfies {\localimplieslocal} at $y$ as well: see Proposition~\ref{prop:1imp1_implies_locimploc_at_smooth} below.
%
Theorem~\ref{thm:oneimpliesone_char} yields the following necessary, and quite restrictive, condition for {\oneimpliesone}.
\begin{corollary}\label{cor:oneimpliesone_nec_cond}
Unless \emph{all} tangent cones of $\calX$ are linear spaces, no smooth lift for $\calX$ satisfies {\oneimpliesone}.
%$\calX$ has a smooth lift satisfying {\oneimpliesone} only if all its tangent cones are linear spaces.
\end{corollary}
Corollary~\ref{cor:oneimpliesone_nec_cond} shows that {\oneimpliesone} usually does not hold at preimages of nonsmooth points of $\calX$ (see Definition~\ref{def:smth_locus}), whose tangent cones are rarely linear, so all lifts may introduce spurious critical points on $\calM$. 
Table~\ref{tab:lifts} gives several examples of popular lifts of nonsmooth sets violating {\oneimpliesone}. 
Corollary~\ref{cor:oneimpliesone_nec_cond} reveals that no smooth lift of these sets can satisfy {\oneimpliesone}. 
%Thus, we almost always have to check {\twoimpliesone} as well.
This is our main motivation for studying {\twoimpliesone}.

Our characterization of {\twoimpliesone} is more involved. We therefore also give sufficient conditions that are easier to check in many examples, and a necessary condition that is easier to refute in others.
\begin{theorem}\label{thm:2implies1_chain}
Let $\varphi\colon\calM\to\calX$ be a smooth lift and fix $y\in\calM$. We have the following chain of implications for {\twoimpliesone}, where the cones $W_y$ and $B_y$ in $\calE$ are defined in Definitions~\ref{def:W_y} and~\ref{def:A_B_sets}, respectively, and are expressed in terms of $\Lmap_y$ and $\Qmap_y$ in Proposition~\ref{prop:2implies1_with_Qmap}.
\begin{align*}
		&\T_x \calX \subseteq \im \Lmap_y + \Qmap_y(\ker\Lmap_y)\\
		\iff& \T_x \calX = \im \Lmap_y + \Qmap_y(\ker\Lmap_y)\\
		\implies& B_y^* \subseteq (\T_x \calX)^* \\
		\implies& W_y \subseteq (\T_x \calX)^* \\
		\iff& \varphi \textrm{ satisfies {\twoimpliesone} at } y \\
		\implies& (\im \Lmap_y)^\perp \cap (\Qmap_y(\T_y\calM))^* \subseteq (\T_x \calX)^*.
	\end{align*}
\end{theorem}
We show that the first sufficient condition above is not necessary in Example~\ref{ex:A_suff_cond_for_LR}, and that the necessary condition is not sufficient in Example~\ref{ex:nec_cond_isnt_suff}. We conjecture that the second sufficient condition is not necessary either, see Conjecture~\ref{conj:B_suff_cond} below.

In the remainder of this section, we prove the above theorems and explain how to compute the quantities appearing in them. We then apply them to a variety of examples in Section~\ref{sec:examples}. 

%\input{Lifts/approx_crit_pts}

